SwarmMesh: A Distributed Data Structure for Cooperative Multi-Robot Applications

We present an approach to the distributed storage of data across a swarm of mobile robots that forms a shared global memory. We assume that external storage infrastructure is absent, and that each robot is capable of devoting a quota of memory and bandwidth to distributed storage. Our approach is motivated by the insight that in many applications data is collected at the periphery of a swarm topology, but the periphery also happens to be the most dangerous location for storing data, especially in exploration missions. Our approach is designed to promote data storage in the locations in the swarm that best suit a specific feature of interest in the data, while accounting for the constantly changing topology due to individual motion. We analyze two possible features of interest: the data type and the data item position in the environment. We assess the performance of our approach in a large set of simulated experiments. The evaluation shows that our approach is capable of storing quantities of data that exceed the memory of individual robots, while maintaining near-perfect data retention in high-load conditions.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Distributed Hash Tables ?}

\textbf{Distributed key partitioning}
Explain general idea and give a few examples (Chord, Pastry) ? Also, structured vs unstructured ?

\textbf{Overlay network and routing} 
Explain general idea and give a few examples (Chord, Pastry) ? Also, structured vs unstructured ?

% \begin{figure}[h]
%     \centering
%     \includegraphics[height=5cm]{DistributedHashTable.png}
%     \caption{Make better principle diagram with ID Space (key-partitioning), hashing of data into keys, routing to node for entry storage}
%     \label{fig:my_label}
% \end{figure}

% \subsection{Q-Routing}
% \cite{Boyan1994}, \cite{KumarSharma2018}
% $Q_x(d, y)$

% $$ \Delta Q_x(d, y) = \eta (q + s + t - Q_x(d, y))$$

\subsection{CAP Theorem ?}

